Relational Action Bases: Formalization, Effective Safety Verification, and Invariants (Extended Version)

Modeling and verification of dynamic systems operating over a relational representation of states are increasingly investigated problems in AI, Business Process Management, and Database Theory. To make these systems amenable to verification, the amount of information stored in each relational state needs to be bounded, or restrictions are imposed on the preconditions and effects of actions. We introduce the general framework of relational action bases (RABs), which generalizes existing models by lifting both these restrictions: unbounded relational states can be evolved through actions that can quantify both existentially and universally over the data, and that can exploit numerical datatypes with arithmetic predicates. We then study parameterized safety of RABs via (approximated) SMT-based backward search, singling out essential meta-properties of the resulting procedure, and showing how it can be realized by an off-the-shelf combination of existing verification modules of the state-of-the-art MCMT model checker. We demonstrate the effectiveness of this approach on a benchmark of data-aware business processes. Finally, we show how universal invariants can be exploited to make this procedure fully correct.

==> universal-abs.tex <==
% !TEX root =  main.tex

\section{Eliminating Universal Guards from \uras{s}}
\label{sec:stopping}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SRlast: as asked by one reviewer, I have changed the symbol of the
%%% second mapping from ^+ to \hat for uniformity with the first
%%% \tilde...  I have tried to do the replacement uniformly in the
%%% whole section, but please check if some occurrences of ^+ are
%%% still there!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!hp] 
  \centering
  %%% SRlast: I have added the \small command below in order to make
  %%% the table fit the page... does it look readable?  I have also
  %%% moved on the left the two arrows of the mapping as suggested by
  %%% one of the reviewers...
  \small
  \caption{\label{tab:transformation1}Definitions of the mapping $(\tilde{\cdot})$ %% for introducing failures and eliminating global conditions from guards, respectively.
  }
   \begin{adjustwidth}{-1cm}{}
  \begin{tabular}{rc}
    \\
  \begin{minipage}{.1425\textwidth}
    Original universal RAS $\mathcal{S}$ and unsafe formula $\upsilon$
  \end{minipage} &
  \begin{tabular}{r|c|}
    \cline{2-2}
    (a) & $\Sigma, T, \ext{\Sigma}$  \\ \cline{2-2}
    (b) &  $\ux= x_1,..., x_n$ $\ua=a_1, ..., a_m$  \\ \cline{2-2}
    (c) & $\upsilon(\ux,\ua) := \exists \ue \; \phi(\ue, \ux, \ua)$  \\ \cline{2-2}
    (d) & $\iota(\ux, \ua) := (\bigwedge_{i=1}^n x_i= c_i) \land (\bigwedge_{j=1}^m a_j =\lambda y. d_j)$  \\ \cline{2-2}
    (e) & $\begin{array}{l}
      \mathcalligra{t}\mathcalligra{r}_{\ell}(\ux,\ua,\ux',\ua') := \exists \ue,\ud\,\left(
        \begin{array}{l}
          \gamma(\ue, \ud, \ux,\ua) \wedge \forall k\, \gamma_u(k, \ue,\ud, \ux,\ua)\\
           \wedge\bigwedge_i x'_i= F_i(\ue,\ud, \ux,\ua) \\
       \wedge \bigwedge_j a'_j=\lambda y. G_j(y,\ue, \ud, \ux,\ua)
      \end{array}
      \right) \\
      \begin{array}{l}
        \mbox{where } H(y,\ue, \ud, \ux,\ua) := ~ 
        \mbox{\tt case of }  \{ \\
        \begin{array}{rcl}
          \quad\quad\quad\quad\quad \kappa^{H}_1(y,\ue, \ud, \ux,\ua)  &:&  t^{H}_1(y,\ue, \ud, \ux,\ua) \\
          \quad\quad\quad\quad\quad \cdots && \\
          \quad\quad\quad\quad\quad \kappa^{H}_s(y,\ue, \ud, \ux,\ua) &:&  t^{H}_s(y,\ue, \ud, \ux,\ua) \quad \} \\
        \end{array}  \\
        \mbox{with }  H \in  \{ F_i, G_j \}
      \end{array}
    \end{array}$ \\ \cline{2-2}
    (f) & 
    $\tau(\ux,\ua,\ux',\ua') := \bigvee_{\ell=1}^r \mathcalligra{t}\mathcalligra{r}_{\ell}(\ua,\ua')$
    \\ \cline{2-2}
  \end{tabular} \\
  \multicolumn{1}{c}{\rotatebox{-90}{$\mathbf{\longmapsto}$} \raisebox{-.35cm}{$(\tilde{\cdot})$}} &
  \\
  \begin{minipage}{.1425\textwidth}
    Intermediate Universal RAS $\tilde{\mathcal{S}}$ and unsafe formula
     $\tilde{\upsilon}$
  \end{minipage} &
  \begin{tabular}{r|c|}
    \cline{2-2}
    (a) & $\Sorts{\tilde{\Sigma}}:= \Sorts{\Sigma} \cup \{ \tilde{\mathtt{Elem}}\}$, $\functs{\tilde{\Sigma}}:= \functs{\Sigma} \cup \{ \mathtt{t} ,\mathtt{f} \}$,
          $\tilde{T}:= T\cup \{\mathtt{t}\neq \mathtt{f}\}$, $\ext{\tilde{\Sigma}}:= \ext{\Sigma}$ \\ \cline{2-2}
    (b) & $\tilde{\ux}:=\ux$, $\tilde{\ua}:=\ua, a_{m+1}$ where $a_{m+1}$ is new
            \\ \cline{2-2}
%%sg  ho messo in modo esplicito che quella è solo una abbreviazione
        & for $\ue:=e_1, ..., e_k$, the notation ${\tt A}(\ui)$ abbreviates $\bigwedge_{\ell=1}^k (a_{m+1}[e_{\ell}] = \mathtt{t})$ 
           \\ \cline{2-2}
    (c) & $\tilde{\upsilon}(\tilde{\ux},\tilde{\ua}) := 
            \exists \ue \;({\tt A}(\ue)\wedge \phi(\ue, \ux,\ua))$
          \\ \cline{2-2}
    (d) & $\tilde{\iota}(\tilde{\ux},\tilde{\ua}) := (\bigwedge_{i=1}^n x_i= c_i) \land  \forall \ue \;({\tt A}(\ue)\Rightarrow
          (\bigwedge_{j=1}^m a_j[e] = d_j))
%%sg   non serve a nulla supporre che non ci siano processi crashed al'inizio, tanto vale non mettere per semplicità questa assunzione
     %%inoltre se si mette che  non ci sono processi crashed all'inizio va cambiato l'enunciato del lemma 5.4
     %\wedge \forall i.{\tt A}(i)
        $  
                         \\ \cline{2-2}
    (e) & $\begin{array}{l}
      \tilde{\mathcalligra{t}\mathcalligra{r}}_{\ell}(\tilde{\ux},\tilde{\ua},\tilde{\ux}',\tilde{\ua}') := \exists \ue,\ud\,\left(
      \begin{array}{l}
        {\tt A}(\ue)\wedge \gamma(\ue, \ud,\ux,\ua) \wedge \\
       \wedge  \forall k\, ({\tt A}(k)\Rightarrow \gamma_u( k, \ue,\ud, \ux, \ua)) \wedge \\
%FA - RW1 - page 13: $a'_{s+1} = a_s$ should be $a'_{s+1} = a_{s+1}$
         \wedge\bigwedge_i x'_i= F^{\mathtt{A}}_i(\ue,\ud, \ux,\ua) \wedge \\
       \wedge \bigwedge_j a'_j=\lambda y. G^{\mathtt{A}}_j(y,\ue, \ud, \ux,\ua,a_{m+1}[y])\\
        \wedge a_{m+1}'=a_{m+1}
      \end{array}
      \right)\\
      \begin{array}{l}
     \mbox{where } F^{\mathtt{A}}_i(\ue,\ud,\ux,\ua):= F_i(\ue,\ud,\ux,\ua)  \\
     %, \beta) := ~ 
    %  \mbox{\tt case of }  \{ \\
     % \begin{array}{rcl}
     % \quad\quad\quad\quad\quad \kappa^{F_i}_1(\ue,\ud,\ux,\ua)\wedge \beta = \mathtt{t} &:&  t^{F_i}_1(y, \ue,\ud,\ux,\ua) \\
     % \quad\quad\quad\quad\quad \cdots && \\
     % \quad\quad\quad\quad\quad \kappa^{F_i}_s(\ue,\ud,\ux,\ua)\wedge \beta = \mathtt{t} &:&  t^{F_i}_s(\ue,\ud,\ux,\ua) \\
     % \quad\quad\quad\quad\quad \beta = \mathtt{f}  &:& a_i[e]  \quad \}
     % \end{array} \\
      \mbox{and } G^{\mathtt{A}}_j(y, \ue,\ud,\ux,\ua, \beta) := ~ 
      \mbox{\tt case of }  \{ \\
      \begin{array}{rcl}
      \quad\quad\quad\quad\quad \kappa^{G_j}_1(y, \ue,\ud,\ux,\ua)\wedge \beta = \mathtt{t} &:&  t^{G_j}_1(y, \ue,\ud,\ux,\ua) \\
      \quad\quad\quad\quad\quad \cdots && \\
      \quad\quad\quad\quad\quad \kappa^{G_j}_s(y, \ue,\ud,\ux,\ua)\wedge \beta = \mathtt{t} &:&  t^{G_j}_s(y, \ue,\ud,\ux,\ua) \\
      \quad\quad\quad\quad\quad \beta = \mathtt{f}  &:& a_j[y]  \quad \}
        \end{array} \\
          \end{array} \\
     \end{array}$ \\ \cline{2-2}
    (e$'$) & 
    $\tilde{\mathcalligra{t}\mathcalligra{r}}_{r+1}(\tilde{\ux},\tilde{\ua},\tilde{\ux}',\tilde{\ua}') := 
      \exists e \;({\tt A}(e)\wedge \ux'=\ux \wedge \ua'=\ua \wedge  
                   a_{m+1}'= \mathtt{upd}(a_{m+1}, e, \mathtt{f}))$
    \\ \cline{2-2}
    (f) & 
    $\tilde{\tau}(\tilde{\ux},\tilde{\ua},\tilde{\ux}',\tilde{\ua}') := 
      \bigvee_{\ell=1}^{r+1} \tilde{\mathcalligra{t}\mathcalligra{r}}_{\ell}(\tilde{\ux},\tilde{\ua},\tilde{\ux}',\tilde{\ua}')$
    \\ \cline{2-2}
  \end{tabular}
    \end{tabular}
     \end{adjustwidth}
\end{table}


  \begin{table}[!hp] 
  \centering
  %%% SRlast: I have added the \small command below in order to make
  %%% the table fit the page... does it look readable?  I have also
  %%% moved on the left the two arrows of the mapping as suggested by
  %%% one of the reviewers...
  \small
  \caption{\label{tab:transformation2}Definitions of the mapping $(\hat{\cdot})$ %% for introducing failures and eliminating global conditions from guards, respectively.
  }
   \begin{adjustwidth}{-1cm}{}
  \begin{tabular}{rc}
    \\
    \begin{minipage}{.1425\textwidth}
    Intermediate universal RAS $\tilde{\mathcal{S}}$ and unsafe formula
    %unsafe states 
    $\tilde{\upsilon}$
  \end{minipage} &
  \begin{tabular}{r|c|}
    \cline{2-2}
    (a) & $\Sorts{\tilde{\Sigma}}:= \Sorts{\Sigma} \cup \{ \tilde{\mathtt{Elem}}\}$, $\functs{\tilde{\Sigma}}:= \functs{\Sigma} \cup \{ \mathtt{t} ,\mathtt{f} \}$,
          $\tilde{T}:= T\cup \{\mathtt{t}\neq \mathtt{f}\}$, $\ext{\tilde{\Sigma}}:= \ext{\Sigma}$ \\ \cline{2-2}
    (b) & $\tilde{\ux}:=\ux$, $\tilde{\ua}:=\ua, a_{m+1}$ where $a_{m+1}$ is new
            \\ \cline{2-2}
%%sg  ho messo in modo esplicito che quella è solo una abbreviazione
        & for $\ue:=e_1, ..., e_k$, the notation ${\tt A}(\ui)$ abbreviates $\bigwedge_{\ell=1}^k (a_{m+1}[e_{\ell}] = \mathtt{t})$ 
           \\ \cline{2-2}
    (c) & $\tilde{\upsilon}(\tilde{\ux},\tilde{\ua}) := 
            \exists \ue \;({\tt A}(\ue)\wedge \phi(\ue, \ux,\ua))$
          \\ \cline{2-2}
    (d) & $\tilde{\iota}(\tilde{\ux},\tilde{\ua}) := (\bigwedge_{i=1}^n x_i= c_i) \land  \forall \ue \;({\tt A}(\ue)\Rightarrow
          (\bigwedge_{j=1}^m a_j[e] = d_j))
%%sg   non serve a nulla supporre che non ci siano processi crashed al'inizio, tanto vale non mettere per semplicità questa assunzione
     %%inoltre se si mette che  non ci sono processi crashed all'inizio va cambiato l'enunciato del lemma 5.4
     %\wedge \forall i.{\tt A}(i)
        $  
                         \\ \cline{2-2}
    (e) & $\begin{array}{l}
      \tilde{\mathcalligra{t}\mathcalligra{r}}_{\ell}(\tilde{\ux},\tilde{\ua},\tilde{\ux}',\tilde{\ua}') := \exists \ue,\ud\,\left(
      \begin{array}{l}
        {\tt A}(\ue)\wedge \gamma(\ue, \ud,\ux,\ua) \wedge \\
       \wedge  \forall k\, ({\tt A}(k)\Rightarrow \gamma_u( k, \ue,\ud, \ux, \ua)) \wedge \\
%FA - RW1 - page 13: $a'_{s+1} = a_s$ should be $a'_{s+1} = a_{s+1}$
         \wedge\bigwedge_i x'_i= F^{\mathtt{A}}_i(\ue,\ud, \ux,\ua) \wedge \\
       \wedge \bigwedge_j a'_j=\lambda y. G^{\mathtt{A}}_j(y,\ue, \ud, \ux,\ua,a_{m+1}[y])\\
        \wedge a_{m+1}'=a_{m+1}
      \end{array}
      \right)\\
      \begin{array}{l}
       \mbox{where } F^{\mathtt{A}}_i( \ue,\ud,\ux,\ua):=F_i( \ue,\ud,\ux,\ua)  \\
       %, \beta) := ~ 
     % \mbox{\tt case of }  \{ \\
     % \begin{array}{rcl}
     % \quad\quad\quad\quad\quad \kappa^{F_i}_1(\ue,\ud,\ux,\ua)\wedge \beta = \mathtt{t} &:&  t^{F_i}_1(\ue,\ud,\ux,\ua) \\
     % \quad\quad\quad\quad\quad \cdots && \\
    %  \quad\quad\quad\quad\quad \kappa^{F_i}_s(\ue,\ud,\ux,\ua)\wedge \beta = \mathtt{t} &:&  t^{F_i}_s(\ue,\ud,\ux,\ua) \\
    %  \quad\quad\quad\quad\quad \beta = \mathtt{f}  &:& a_i[e]  \quad \}
    %  \end{array} \\
      \mbox{and } G^{\mathtt{A}}_j(y, \ue,\ud,\ux,\ua, \beta) := ~ 
      \mbox{\tt case of }  \{ \\
      \begin{array}{rcl}
      \quad\quad\quad\quad\quad \kappa^{G_j}_1(y, \ue,\ud,\ux,\ua)\wedge \beta = \mathtt{t} &:&  t^{G_j}_1(y, \ue,\ud,\ux,\ua) \\
      \quad\quad\quad\quad\quad \cdots && \\
      \quad\quad\quad\quad\quad \kappa^{G_j}_s(y, \ue,\ud,\ux,\ua)\wedge \beta = \mathtt{t} &:&  t^{G_j}_s(y, \ue,\ud,\ux,\ua) \\
      \quad\quad\quad\quad\quad \beta = \mathtt{f}  &:& a_j[y]  \quad \}
      \end{array} \\
       %\mbox{with } H \in  \{ F_i, G_j \}
      \end{array}
     \end{array}$ \\ \cline{2-2}
    (e$'$) & 
    $\tilde{\mathcalligra{t}\mathcalligra{r}}_{r+1}(\tilde{\ux},\tilde{\ua},\tilde{\ux}',\tilde{\ua}') := 
      \exists e \;({\tt A}(e)\wedge \ux'=\ux \wedge \ua'=\ua \wedge  
                   a_{m+1}'= \mathtt{upd}(a_{m+1}, e, \mathtt{f}))$
    \\ \cline{2-2}
    (f) & 
    $\tilde{\tau}(\tilde{\ux},\tilde{\ua},\tilde{\ux}',\tilde{\ua}') := 
      \bigvee_{\ell=1}^{r+1} \tilde{\mathcalligra{t}\mathcalligra{r}}_{\ell}(\tilde{\ux},\tilde{\ua},\tilde{\ux}',\tilde{\ua}')$
    \\ \cline{2-2}
  \end{tabular}\\
  \multicolumn{1}{c}{\rotatebox{-90}{$\mathbf{\longmapsto}$} \raisebox{-.35cm}{$(\widehat{\cdot})$}} &
  \\
  \begin{minipage}{.1425\textwidth}
    Target (plain) RAS $\widehat{\mathcal{S}}$ and unsafe formula $\widehat{\upsilon}$
  \end{minipage} &
  \begin{tabular}{r|c|}
    \cline{2-2}
    (a) & $\widehat{\Sigma}:=\tilde{\Sigma}$, 
          $\widehat{T}:=\tilde{T}$ and $\ext{\widehat{\Sigma}}:= \ext{\tilde{\Sigma}}$ \\ \cline{2-2} 
    (b) & $\widehat{\ux}:= \tilde{\ux}$, $\widehat{a}:=\tilde{a}$   \\ \cline{2-2}
    (c) & $\widehat{\upsilon}(\widehat{\ux},\widehat{\ua}):=\tilde{\upsilon}(\tilde{\ux},\tilde{\ua})$ \\ \cline{2-2}
    (d) & $\widehat{\iota}(\widehat{\ux},\widehat{\ua}) := \tilde{\iota}(\tilde{\ux},\tilde{\ua})$  \\ \cline{2-2}
    (e) & $\begin{array}{l}
      \widehat{\mathcalligra{t}\mathcalligra{r}}_{\ell}(\widehat{\ux},\widehat{\ua},\widehat{\ux}',\widehat{\ua}') := \exists \ue, \ud\,\left(
      \begin{array}{l}
        {\tt A}(\ue)\wedge \gamma(\ue,\ud,\ux,\ua) \wedge \\
       \wedge  \bigwedge_{k\in \ue} \gamma_u(k,\ue, \ud, \ux, \ua) \\
        \wedge\bigwedge_i x'_i= F^{\mathtt{A},{\forall}}_i(\ue,\ud, \ux,\ua) \wedge \\
       \wedge \bigwedge_j a'_j=\lambda y. G^{\mathtt{A},{\forall}}_j(y,\ue, \ud, \ux,\ua,a_{m+1}[y])\\
        \wedge a_{m+1}'=\lambda y.f^{\mathtt{A},{\forall}}(y,\ue,\ud,\ux,\ua,a_{m+1}[y])
      \end{array}
      \right)\\
      \begin{array}{l}
        \mbox{where } F^{\mathtt{A},{\forall}}_i(\ue,\ud,\ux,\ua) :=   F_i(\ue,\ud,\ux,\ua) \\
   %   \mbox{\tt case of }  \{ \\
   %   \quad\quad\quad\quad\quad
   %   \begin{array}{rcl}
   %     \kappa^{F_i}_1(y,\ue,\ud,\ux,\ua)\wedge 
    %    \beta = \mathtt{t}\wedge \gamma_u(y,\ue,\ud,\ux,\ua)  &:&  t^{F_i}_1(y,\ue,\ud,\ux,\ua) \\
   %     \cdots && \\
   %      \kappa^{F_i}_s(y,\ue,\ud,\ux,\ua)\wedge 
    %    \beta = \mathtt{t}\wedge  \gamma_u(y,\ue,\ud,\ux,\ua) &:&  t^{F_i}_s(y,\ue,\ud,\ux,\ua) \\
   %      \beta = \mathtt{f}\vee \neg  \gamma_u(y,\ue,\ud,\ux,\ua)  &:&  a_j[y]~~ \} \\              \end{array}\\
          \mbox{and } G^{\mathtt{A},{\forall}}_j(y,\ue,\ud,\ux,\ua, \beta) := 
      \mbox{\tt case of }  \{ \\
      \quad\quad\quad\quad\quad
      \begin{array}{rcl}
        \kappa^{G_j}_1(y,\ue,\ud,\ux,\ua)\wedge 
        \beta = \mathtt{t}\wedge  \gamma_u(y,\ue,\ud,\ux,\ua)  &:&  t^{G_j}_1(y,\ue,\ud,\ux,\ua) \\
        \cdots && \\
         \kappa^{G_j}_s(y,\ue,\ud,\ux,\ua)\wedge 
        \beta = \mathtt{t}\wedge  \gamma_u(y,\ue,\ud,\ux,\ua) &:&  t^{G_j}_s(y,\ue,\ud,\ux,\ua) \\
         \beta = \mathtt{f}\vee \neg  \gamma_u(y,\ue,\ud,\ux,\ua)  &:&  a_j[y]~~ \} \\              \end{array}\\
      % \mbox{with } H \in  \{ F_i, G_j \}, \\
       \mbox{and }         f^{\mathtt{A},{\forall}}(y,\ue,\ud,\ux,\ua,\beta) :=
        {\tt if}~(\beta=\mathtt{f} \vee \neg  \gamma_u(y,\ue,\ud,\ux,\ua))
        ~{\tt then}~\mathtt{f}~{\tt else}~\beta
      \end{array}
     \end{array}$ \\ \cline{2-2}
    (e$'$) & 
    $\widehat{\mathcalligra{t}\mathcalligra{r}}_{r+1}(\widehat{\ux},\widehat{\ua},\widehat{\ux}',\widehat{\ua}') := \tilde{\mathcalligra{t}\mathcalligra{r}}_{r+1}(\widehat{\ux},\widehat{\ua},\widehat{\ux}',\widehat{\ua}')$
     \\ \cline{2-2}
    (f) & 
    $\widehat{\tau}(\widehat{\ux},\widehat{\ua},\widehat{\ux}',\widehat{\ua}') := 
      \bigvee_{\ell=1}^{r+1} \widehat{\mathcalligra{t}\mathcalligra{r}}_{\ell}(\widehat{\ux},\widehat{\ua},\widehat{\ux}',\widehat{\ua}')$
    \\ \cline{2-2}
  \end{tabular} 
  \end{tabular}
     \end{adjustwidth}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SRlast: I have tried to simplify the beginning of the section
%%% since the formula \ref{eq:transition3} has been moved to the table
%%% where all the assumptions have been put for ease of reference...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%As illustrated in Section~\ref{subsec:running-the-problem}, 
In general, it is difficult to automate $\mathsf{BReach}$ in the general case of universal RASs, i.e. when the transition formulae
$\mathcalligra{t}\mathcalligra{r}$ contain a universal guard $\gamma_u$ (cf. Formula~\eqref{eq:trans1}). %see \textbf{(wHF3)} in
%Table~\ref{tab:assumptions} for the definition.
%% mechanize the backward reachability procedure of
%% Figure~\ref{fig:reach-algo} in presence of transitions of the form
%% \begin{equation}
%%   \label{eq:transition3}
%%   \exists \ui\,(\phi_L(\ui, a[\ui]) \wedge 
%%                 \forall k\, \psi(\ui, k, a[\ui], a[k])\wedge 
%%                 a'=\lambda j. F(\ui, a[\ui], j, a[j])) ;
%% \end{equation}
%% these formulae are called \emph{universally guarded transition
%%   formulae in functional form}.  
The main problem is  that, in order to symbolically execute Formula~\eqref{eq:trans1}, we need
%% the need to symbolically execute (\ref{eq:transition3}), we need
to check whether the the universal guards $\gamma_u$ %of a disjunct of the form
 in $\tau$ holds for all the entries of an artifact relation
% FA - RW2 - composing the system --> comprising the system  
%comprising the system 
(i.e.\ a finite but unknown number of tuples)
rather than on a bounded number as it is the case for the (plain) guard $\gamma$.
%% sg questo pezzo è stato riscritto: l'idea è di non presentare le
%% trasformazioni come puri giochetti per far tornare i conti ma di
%% motivarle
To solve this problem, the key idea is to design a syntactic
transformation of the Universal RAS 
%% is underlying our transformations for dealing with the above
%% transitions can be summarized as follows: 
so as to obtain a sufficiently precise \emph{abstraction} that
preserves the safety properties.  The abstraction is inspired by an analogous transformation introduced in \cite{jsat}, where this transformation is interpreted in a semantic way. 
In fact, in the context of \cite{jsat}, indexes $\ue$ are not interpreted as entries of artifact relations as we do here, but as (identifiers of) processes. 
When dealing with real processes that should follow a protocol, it is usually licit  to
adopt the following \emph{(stopping) failure model}:
%%% Our failure model is simple: %%%%%%%%%%%%%%%%%%%%%
\emph{processes can crash and crashed
  processes are not permitted to take an active role in the protocol}. In \cite{jsat} it is proved  that, when this model is adopted,  (modulo bisimulation) universally guarded
transitions  can be
% FA - RW2 - replaced by ordinary transitions in functional form (3) --> replaced by transitions in the simple functional form (3)
replaced by transitions not containing universal quantifiers.  Intuitively, this is possible since in the abstracted system processes not satisfying the universal guard are interpreted as crashed, and runs with crashed processes are allowed.

In order to verify Universal RASs, we take inspiration from the results proved in \cite{jsat}.
Although it is not clear how to import the semantical  interpretation of crashing processes into our framework, 
it is still useful to introduce an analogous syntactic transformation for Universal RASs into (plain) RASs. This allows us to perform the safety verification on universal RASs
via the backward reachability procedure bypassing the formal issues due to universal guards. 
%We shall make this
%observation rigorous in the technical developments below.  
We
point out that RAS obtained by this transformation is a more liberal array-based system, i.e., it has more runs than the original system.  As
a consequence, if a set of bad states represented by the unsafe formula $\upsilon$ is shown to be unreachable
for the abstracted system, then it will also be unreachable for the
original system.  %In practice, many common distributed algorithms are
%fault-tolerant and this explains why it is not by chance that our
%approach usually works and produces the desired safety certifications,
%as it is evident from the extensive experiments reported
%in~\cite{lmcs}.

%% sg questa osservazione l'ho tolta perchè è solo una mezza
%% giustificazione (non gioustifica perchè aggiungiamo anche la
%% transizione che manda in crash un processo senza ragione; è vero
%% che potremmo forse togliere questa transizione, ma allora veramente
%% tutto diventa solo formale
% 
% Here, we explain how to find an over-approximation for this
%kind of transition formulae by using an auxiliary variable, say $f$,
%that keeps track of processes violating the global guards and
%eliminating the need to evaluate $\forall k\, \psi(\ui, k, a[\ui],
%a[k])$.  The variable $f$ is an array of Booleans such that $f[i]$ is
%true iff the process $i$ has never violated a global guard $\psi$ of
%any transition.  Indeed, the local guard of the new version of
%(\ref{eq:transition3}) should check that only those processes with $f$
%set to true are considered for the application of the modified
%transition.  The key point is that the resulting transition formula is
%in functional form so that the backward reachability procedure
%$\mathsf{BReach}$ of Figure~\ref{fig:reach-algo} can be mechanized
%along the lines of Section~\ref{sec:array}.  
%
%
%%sg questo pezzo è stato rimesso più o meno con le stesse parole sopra
%Moreover, the array-based
%system obtained by this transformation is more liberal, i.e.\ it has
%more runs than the original system.  As a consequence, if a set of bad
%states $U$ is shown to be unreachable for the more liberal system,
%then it will also be unreachable for the original system.  We will see
%that for the class of array-based systems considered in this paper,
%also the converse holds.

%%sg  frase spostata sotto
%In Table~\ref{tab:transformation}, the precise definition of the
%purely syntactic transformation sketched above is given.  
%Let $T_I$ and $T_E$ be theories,

Let $\cSi$ be a Universal RAS as in Section~\ref{sec:artifact}, and $\upsilon$ an unsafe formula %$\exists^I$-formula (
describing a set of unsafe
states.
%) satisfying the assumptions \textbf{(HT1)}, \textbf{(HT2)},
%\textbf{(HF1)}, \textbf{(HF2)}, and 
%%% SRlast: I have simplified the following sentence because of the
%%% newly introduced table recording the assumptions...
%% the following weakened version of
%% \textbf{(HF3)}, identified by 
%\textbf{(wHF3)} in Table~\ref{tab:assumptions}.
%% : $\tau$ is a disjunction
%% of formulae of the form (\ref{eq:transition2}) or
%% (\ref{eq:transition3}).
%% sg ripetizione inutile
%, i.e.\ transition formulae whose guards can be
%seen as conjunctions of a local (existential) and, possibly, a global
%(universal) condition.  
%%
%%sg spiegazione più estesa
%
To make clearer the formal definition of the syntactic transformation, we
split it in two different maps, namely $(\tilde{\cdot{}})$ and
$(\hat{\cdot{}})$, defined on safety problems, i.e.\ pairs of a system and an unsafe formula.
%%sg ripetizione
%It is easy to see that such pairs identify safety problems as defined
%in Section~\ref{sec:array-based-sys}.  
The first map $(\tilde{\cdot{}})$ \emph{introduces ``failures'' for some indexes} and
transforms a Universal RAS $(\cSi,\upsilon)$ into what we call an \emph{intermediate Universal RAS $(\tilde{\cSi},\tilde{\upsilon})$}. The last model is an instance Universal RAS, since it still contains universal guards.
% sg questo dettaglio è messo sotto by adding an auxiliary variable
% and relativizing all quantifiers.
The second map $(\hat{\cdot{}})$ \emph{removes the universal
  guards} and transforms $(\tilde{\cSi},\tilde{\upsilon})$ to a (plain) RAS
$(\widehat{\cSi},\widehat{\upsilon})$. The last is a plain RAS since it does not contain universally quantified guards anymore.
%%sg questo dettaglio è spostato sotto
% by eliminating universal guards and suitably modifying the updates
% of the transitions of the form (\ref{eq:transition3}) while leaving
% (almost) unmodified those of the form (\ref{eq:transition2}).
%
%%% SR: RIFRASATO QUELLO CHE SEGUE
% We describe each step in more details below and during our exposition
% we refer to the relevant lines of Table~\ref{tab:transformation},
% where our purely syntactic transformations are fully reported.
The two maps are formally shown in Table~\ref{tab:transformation1} and in Table~\ref{tab:transformation2}, respectively. In the following, we comment in details on these transformations.

\noindent
{\textbf{First Step}: \framebox{$(\cSi,\upsilon) \longmapsto
    (\tilde{\cSi},\tilde{\upsilon})$}.}  The technique for introducing the
``failure version'' of $(\cSi,\upsilon)$ consists in adding an auxiliary variable
and then in relativizing all quantifiers to a predicate ${\tt A}(\ue)$ representing the
``non-failed/non-disappeared'' entries. This is achieved in the following way.
\begin{description}
 \item[-] In (a), we add a new sort $\tilde{\mathtt{ELEM}}$ with two constant
symbols $\mathtt{t}$ and $\mathtt{f}$ to $\functs{\Sigma}$ of the DB schema $\tup{\Sigma, T}$ so that the models of $T$ are
expanded in such a way that $\tilde{\mathtt{ELEM}}$ is interpreted as a
set of two elements, and $\mathtt{t}$ and $\mathtt{f}$ are mapped to
distinct elements of this set.
%%sg rewording
% FA - RW2 - p.14, comment to (a). You can safely remove the phrase in parentheses ("in practice, we...").
%(in practice, we just add a copy of the Boolean
%values $\mathit{true}$ and $\mathit{false}$, respectively).
\item[-]  In (b),
the auxiliary artifact component  $a_{m+1}$  is added to the original artifact components $\ua$ of
the system and the resulting tuple of variables, comprising all the artifact components of the new system, is denoted with
$\tilde{\ua}$.  The abbreviation ${\tt A}(\ue)$ is introduced in order
to identify the conjunction of equalities between the terms 
%%sg-last ho messo l'indice s+1, c'era $a[\ui]$
$a_{m+1}[\ue]$
%%ssg aggiunta spiegazione
%
and the constant $\mathtt{t}$. This predicate is essential in order to relativize all the universal quantifiers to ``non-failed'' entries. %the formula ${\tt A}(e_{\ell})$ means
%that ``$e_{\ell}$ is not crashed''.
\item[-] In (c), the existential quantifier of the safety formula  $\upsilon$ is
  ``relativized'' with respect to ${\tt A}$.
  %% sg non serve a nulla supporre che non ci siano processi crashed
  %% al'inizio, tanto vale non mettere per semplicità questa
  %% assunzione
  % In (d), besides making the relativization of the universal
  % quantifier of $I$, the initial value of auxiliary values is
  % constrained to be $\mathtt{t}$ for every index.
\item[-] In (d), the universal quantifier of the initial formula $\iota$ is also relativized with respect to ${\tt A}$.
\item[-] In (e), the existential and universal quantifiers of the
  transition formula are relativized with respect to ${\tt A}$;
  similarly, the case-defined functions of the updates are also
  relativized so as to modify
  %% sg rewording
  % only the values of the arrays $a$ with the auxiliary variable
  % $a_{s+1}$ set to $\mathtt{t}$.
  the values of the artifact components $\ua$ only whenever the auxiliary artifact component
  $a_{m+1}$ is set to $\mathtt{t}$.
  % 
  % 
  Formally, this is achieved by adding an extra parameter $\beta$ to the
  case-defined function and creating a new partition by splitting on
  its two possible values (either $\mathtt{t}$ or $\mathtt{f}$) and
  then distributing over $\kappa^{H}_1, ..., \kappa^{H}_k$.  According to this
  transformation, formulae %of the form~\eqref{eq:transition2},
  %obtained from 
  $\mathcalligra{t}\mathcalligra{r}(\ux,\ua, \ux', \ua')$ from the definition of RASs (Section~\ref{sec:artifact}) %in Table~\ref{tab:transformation1} by taking
  %$\psi$ to be equivalent to $\mathit{true}$, 
  are mapped to
  \begin{equation}
    \label{eq:transition2t}
    \exists \ue,\ud\,\left(
      \begin{array}{l}
        {\tt A}(\ue)\wedge \gamma(\ue, \ud,\ux,\ua)  
       \wedge  \forall k\, ({\tt A}(k)\Rightarrow \gamma_u( k, \ue,\ud, \ux, \ua)) \wedge \\
%FA - RW1 - page 13: $a'_{s+1} = a_s$ should be $a'_{s+1} = a_{s+1}$
        \bigwedge_i x'_i= F^{\mathtt{A}}_i(\ue,\ud, \ux,\ua,a_{m+1}[e]) \wedge 
        \bigwedge_j a'_j=\lambda y. G^{\mathtt{A}}_j(y,\ue, \ud, \ux,\ua,a_{m+1}[y])\\
        \wedge \, {} a_{m+1}'=a_{m+1}
      \end{array}
       \right)\\
  \end{equation}
  where $F^{\mathtt{A}}_i$ and $G^{\mathtt{A}}_j$ are case-defined functions as defined in Table~\ref{tab:transformation1}
  %and those of the form~\eqref{eq:transition3} to
%  \begin{equation}
   % \label{eq:transition3t}
   % \exists \ui\,\left(
  %    \begin{array}{l}
  %      {\tt A}(\ui)\wedge \phi_L(\ui, a[\ui]) \wedge 
 %       \forall k\, ({\tt A}(k)\Rightarrow \psi(\ui, k, a[\ui], a[k])) \wedge\\
  %      \tilde a'=\lambda j. \tilde F(\ui, \tilde a[\ui], j, \tilde a[j])
  %    \end{array}
    %  \right) ,
%  \end{equation}
  % sg typos
  %where $\tilde a'=\lambda j. \tilde F(\ui, \tilde a[\ui], j, \tilde
  %a[j])$ abbreviates $a'=\lambda j. F_{\mathtt{A}}(\ui, a[\ui], j,
  %a[j], a_{s+1}[j]) \wedge a_{s+1}'=a_{s+1}$.
  %
 % \footnote{In
%% FA - RW2 - "In Table 2, we made some notational simplifications that deserve a comment."
%    Table~\ref{tab:transformation}, we made some notational simplifications
%    that deserve a comment.  First, in the lines marked
%    with (e), the length of the tuple $\ui$ as well as the vectors of
%    function symbols $F, F_{\tt A}, \dots$ should depend on $\ell$; we
%    omitted this dependence to
 %   % FA - RW2 - avoid notation overhead --> avoid the notation overhead
  %  avoid the notation overhead.  Second, since
  %  the $F$'s are vectors (having $s$-components, like the $a$'s), the
  %  tuple $o_1, \dots, o_k$ is a tuple of vectors of terms, each of
 %   which having $s$-components.  (All this is consistent with our
 %   policy to use non-underlined names for tuples of expressions
 %   having fixed length $s$.)  Third, since any two $T$-partitions
 %   have a common refinement, one can freely assume that the
%    $T$-partition used in the definitions of the $F$'s is the same for
 %   all the $s$-components of the vector $F$.} 
    Notice that the value
  of $a_{m+1}$ is not changed by the transition $\tilde{\mathcalligra{t}\mathcalligra{r}}_{\ell}$.
\item[-]
  %% sg aggiunta spiegazione
  In (e$'$), we formalize the fact that an entry can ``disappear'' at any
  time:  we disregard here what is the real interpretation of this phenomenon, it is just instrumental to give an intuition of what the abstraction does. Formally, what we do is to add the $(r+1)$-transition $\tilde{\mathcalligra{t}\mathcalligra{r}}_{r+1}$, which leaves the original
  variables in $\ua$ unchanged and non-deterministically changes the
  value of a cell of $a_{m+1}$ from $\mathtt{t}$ to $\mathtt{f}$. The notation $a_{m+1}'= \mathtt{upd}(a_{m+1}, e, \mathtt{f}))$ in Table~\ref{tab:transformation1}
  is an abbreviation for the case-defined function 
%%% SR: eliminato "term" che mi sembra che appesantisca e basta
$\lambda y.(\mathtt{if}~(y=e)~\mathtt{then}~\mathtt{f}~\mathtt{else}
%%sg-last corretto typo, c'era ~a[i])$ 
~a_{m+1}[y])$ 

  %% sg lascerei perdere l'osservazione che segue (c'è già
  %% abbastanza casino)
  % For the sake of uniformity, we have relativized the existential
  % quantifier in $\tilde{t}_{n+1}$ with respect to ${\tt A}$ although
  % this is not strictly necessary.
\item[-]
  %% sg rewording
  Finally, in (f), we construct the new transition formula
  $\tilde{\tau}$ by taking the disjunction of the
  ``relativized'' transition formulae $\tilde{\mathcalligra{t}\mathcalligra{r}}_1, ..., \tilde{\mathcalligra{t}\mathcalligra{r}}_r$
  with the additional disjunct $\tilde{\mathcalligra{t}\mathcalligra{r}}_{r+1}$.
%
\end{description}
%It is not difficult to show that the safety problems $(\cSi,\upsilon)$ and
%$(\tilde{\cSi},\tilde{\upsilon})$ have the same answer provided that $\tau$
%is in functional form (see Proposition~\ref{prop:equiv} in
%Section~\ref{subsec:props-relativization} below).

We will show (Proposition~\ref{prop:preserve-safety} below) that if  $\tilde{\cSi}$ is safe w.r.t.  $\tilde{\upsilon}$,
then also $\cSi$ is safe w.r.t. $\upsilon$. This is due to the fact that $\tilde{\cSi}$ is an abstraction of  $\cSi$ and contains more unsafe traces. Traces in intermediate Universal RASs $\tilde{\cSi}$ that lead to bad states and that cannot be interpreted as 
licit runs in $\cSi$ are called \emph{spurious traces}.

\noindent
{\textbf{Second Step}: \framebox{$(\tilde{\cSi},\tilde{\upsilon}) \longmapsto
    (\widehat{\cSi},\widehat{\upsilon})$}.}
%% sg pezzo lievemente riscritto
% Most of the work has already been done by the mapping
% $(\tilde{\cdot})$ described above.
We now eliminate the universal guards $\gamma_u$. The definition of this map
is simpler than the previous one.
\begin{description}
\item[-] We do not modify further what we already modified in the first step: the DB theory (a), the
  tuple of the artifact variables and the tuple of the artifact components (b), the safety (c) and the initial
  formulae (d), and (e$'$) the additional transition
  non-deterministically updating the auxiliary variable $a_{s+1}$ are all defined as in the First Step.
\item[-] The interesting part of the map  $(\hat{\cdot})$
  % of $(\hat{\cdot})$ 
  is (e), where we to transform the formulae $\tilde{\mathcalligra{t}\mathcalligra{r}}_1, ..., \tilde{\mathcalligra{t}\mathcalligra{r}}_r$ by
  replacing the universally quantified formula $\forall k\, ({\tt
    A}(k)\Rightarrow \gamma_u(k, \ue, \ud, \ux, \ua))$ in the guard by the
  finite conjunction of quantifier-free formulae
  %%% SRlast: I have replaced ``j'' with ``k'' as suggested by one of
  %%% the reviewer since it is easier to match with the universally
  %%% quantified variable in the global guard above... please, check!
  $\bigwedge_{k\in \ue} \gamma_u(k,\ue, \ud, \ux, \ua)$;
  %% sg ho spezzato il periodo per renderlo più leggibile
  in addition, we modify the case-defined function of the updates as
  follows.  First, we update the arrays $\ua$ only in the correspondence of the entries $k$
  such that the auxiliary variable $a_{m+1}[k]$ is set to $\mathtt{t}$ (as
  before) and for which the (removed) universal guard $\gamma_u(k, \ue,
  \ux,\ua)$
  % in the guard
  holds.  Formally, we create a
  new partition by splitting on $\gamma_u(k, \ue, \ud, \ux, \ua)$ and then
  distributing over the intermediate partition $(\kappa^{G_j}_1\wedge
  \beta=\mathtt{t}), ..., (\kappa^{G_j}_k\wedge \beta=\mathtt{t}),
  \beta=\mathtt{f}$.
Furthermore---and most importantly---we force (through the update function $f_{\mathtt{A}}^{\forall}$)
   the value of
  $a_{m+1}[k]$ for those entires $k$ for which $\gamma_u(k,\ue, \ux,\ua)$ 
  does not hold to become $\mathtt{f}$.  %%sg ripetizione (con typo)
 %Notice also that the update
%function for the auxiliary variable $a_{s+1}$ is such that given a
%certain index $j$, the value of $a_{s+1}'[j]$ is set to $\mathtt{f}$
%if $\psi(i,a[j],j,a_{s+1}[j])$ is not satisfied. 
  According to this transformation, formulae of the
  form~\eqref{eq:transition2t} are mapped to
  \begin{equation}
    \label{eq:transition3tt}
    \exists \ue, \ud\,\left(
      \begin{array}{l}
        {\tt A}(\ue)\wedge \gamma(\ue,\ud,\ux,\ua) \wedge  \bigwedge_{k\in \ue} \gamma_u(k,\ue, \ud, \ux, \ua) 
        \wedge\bigwedge_i x'_i= F^{\mathtt{A},{\forall}}_i(\ue,\ud, \ux,\ua) \wedge \\
       \wedge \bigwedge_j a'_j=\lambda y. G^{\mathtt{A},{\forall}}_j(y,\ue, \ud, \ux,\ua,a_{m+1}[y]) \\
        \wedge a_{m+1}'=\lambda y.f^{\mathtt{A},{\forall}}(y,\ue,\ud,\ux,\ua,a_{m+1}[y])
      \end{array}
      \right)
  \end{equation}
%%sg riga aggiunta
  where $ F^{\mathtt{A},{\forall}}_i, G^{\mathtt{A},{\forall}}_j,f^{\mathtt{A},{\forall}}$ are
  as formally defined in Table~\ref{tab:transformation2}.
\end{description}
We will show (Proposition~\ref{prop:result-abstract} below) that the safety
problems $(\tilde{\cSi},\tilde{\upsilon})$ and $(\widehat{\cSi},\widehat{\upsilon})$
have the same answer. Traces in the RAS $\widehat{\cSi}$ that lead to bad states that cannot be interpreted as
licit runs in the original Universal RAS $\cSi$ are also called \emph{spurious traces}.


% under the assumptions \textbf{(HT1)},
%\textbf{(HT2)}, \textbf{(HF1)}, \textbf{(HF2)}, and \textbf{(wHF3)} of
%Table~\ref{tab:assumptions}.


\subsection{Properties of $(\cSi,\upsilon) \mapsto (\tilde{\cSi},\tilde{\upsilon})$}
\label{subsec:props-relativization}

We recall that when the answer to a safety problem $(\cSi,\upsilon)$ is safe (unsafe), we
say that \emph{$\cSi$ is safe (unsafe, respectively) with respect to
  $\upsilon$}.  

%%sg Ho tolto il capoverso seguente: immagino che ce l'avevo messo io, probabilmente è giustop però 
%% le definizioni che abbiamo dato coprono solo il caso ristretto
%The proof of the following result is easy and does not depend on any
%of the assumptions \textbf{(HT1)}, \textbf{(HT2)}, \textbf{(HF1)},
%\textbf{(HF2)}, and \textbf{(wHF3)} above; it holds for arbitrary
%array-based systems.
\begin{proposition}\label{prop:preserve-safety}
  If $\tilde \cSi$ is safe with respect to $\tilde \upsilon$, then $\cSi$ is
  safe with respect to $\upsilon$.
\end{proposition}
\begin{proof}
  Suppose (by contra-position) that 
  \begin{equation*}
    \iota(\ux^0,\ua^0)\wedge \tau(\ux^0, \ua^0, \ux^0, \ua^1)\wedge \cdots \wedge \tau(\ux^{n-1}, \ua^{n-1}, \ux^n, \ua^n)\wedge
    \upsilon(\ux^k, \ua^k)
  \end{equation*} 
  is satisfiable in a DB-instance $\cM$ under a certain assignment
  ${\tt a}$.  We expand the model $\cM$ to a DB-instance $\tilde \cM$ in the obvious way by interpreting
  $\tilde{\mathtt{ELEM}}$ as a set containing two distinct elements, say
  $0$ and $1$ for the constants $\mathtt{f}$ and $\mathtt{t}$,
  respectively, and interpreting $a_{m+1}$ as a
  (total) functions from $\mathtt{INDEX}^{\cM}$ to $\{0,1\}$.  Then,
  we expand the assignment ${\tt a}$ by assigning to $k$-copies
  $(a_{m+1})_1, \cdots, (a_{m+1})_k$ of the new array variable
  $a_{m+1}$ the array whose constant value is $1$.  In this way, it is
  easy to see that
  \begin{equation*}
    \cM, {\tt a} \models
     \iota(\tilde \ux^0, \tilde \ua^0)\wedge \tau(\tilde \ux^0,\tilde \ua^0, \tilde \ux^1,\tilde \ua^1)\wedge \cdots \wedge
     \tau(\tilde \ux^{n-1}\tilde \ua^{n-1}, \tilde \ux^n, \tilde \ua^n)\wedge \upsilon(\tilde \ux^n, \tilde \ua^n)
   \end{equation*}
   
   ADD NOTATION M,a VDASH
   holds under the assignment $\tt a$ as expanded above and hence
   $\tilde \cSi$ is unsafe with respect to $\tilde \upsilon$.
\end{proof} 
Safety of the intermediate RAS $\tilde{\cSi}$ implies safety of the
original Universal RAS ${\cSi}$.
% FA - RW2 - Remove "Indeed" from "Indeed, the contrary ...".
The contrary is false for arbitrary Universal RASs, because of the presence of spurious unsafe traces in intermediate Universal RASs. %although we


\subsection{Properties of $(\tilde{\cSi},\tilde{\upsilon}) \mapsto
  (\widehat{\cSi},\widehat{\upsilon})$}
\label{subsec:props-for-+}

Consider the transition $\widehat{\univtrans_{\ell}}$ of the target RAS in
Table~\ref{tab:transformation2}: the universal quantifier in the universal guard $\gamma_u$
of $\widehat{\univtrans_{\ell}}$ in the intermediate Universal RAS has been eliminated and
the corresponding values in $a_{m+1}$ of those entries violating the universal guard $\gamma_u$
are set to $\mathtt{f}$.  In this paragraph, we show that the elimination of these
universal conditions from intermediate Universal RASs is without loss of precision
when verifying safety properties. Again, the argument is based on what proved in \cite{jsat}. The reason why $\tilde \cSi$ and
$\widehat{\cSi}$ are equivalent w.r.t. detecting safety is that the transition
$\widehat{\tau}$ can be simulated by finitely many application of the
additional transition $\tilde{\univtrans}_{r+1}$ followed by the application of
$\bigvee_{\ell=1}^n \tilde{\univtrans}_{\ell}$.  In fact, the universal
condition of the guard has been instantiated in $\widehat{\univtrans_{\ell}}$
of Table~\ref{tab:transformation2} only with the entries $k\in \ue$ enabling the
transition. This implies that the transition can fire anyway if the values of
$a_{m+1}$ over the entries violating the universal guard have been set to $\mathtt{f}$ before the transition applies.  To
make this intuition precise, we need to introduce some technical
notions and, in particular, the notion of bisimulation.

Let $\cSi=\tup{\Sigma,T,\ext{\Sigma}, \ux, \ua,  \iota(\ux,\ua),\tau(\ux,\ua,\ux',\ua')}$ be a Universal RAS. A \emph{state} of
$\cSi$ is a pair $(\us,\cM)$ where $\cM$ is a DB-instance and $\us:=\tup{\ux^{\cM},\ua^{\cM}}$.  A \emph{configuration} of $\cSi$ is a state
$(\us,\cM)$ where $\mathcal{S}^\cM$ is a finite set, for every $\mathcal{S} \in \ext{\Sigma}$.  


Below, we write $\cM_{\us}$
to denote the (finite) $\Sigma\cup \ext{\Sigma}$-substructure of $\cM$  generated by $\us$, where $\us$ and $\cM$ are taken from a configuration $\mathcal{C}:=(\us,\cM)$.  The $n$-th
iteration of $\tau(\ux,\ua,\ux',\ua')$ is inductively defined as follows: (i)
$\tau^0(\ux,\ua,\ux',\ua'):=(\ux= \ux')\land (\ua=\ua')$ and (ii) $\tau^{n+1}(\ux,\ua, \ux',\ua'):= \exists
\ux'',\ua'' (\tau(\ux,\ua,\ux'', \ua'') \wedge \tau^n(\ux'',\ua'',\ux', \ua'))$.
\begin{definition} 
  Let  $\cSi_1=\tup{\Sigma,T,\ext{\Sigma}, \ux, \ua,  \iota_1,\tau_1}$ and $\cSi_2=\tup{\Sigma,T,\ext{\Sigma}, \ux, \ua,  \iota_2,\tau_2}$ be two Universal RASs (notice that, in particular, $\cSi_1$ and $\cSi_2$ share the same DB schema $\tup{\Sigma,T}$). A \emph{bisimulation} between them is a relation
  $R$ between configurations $\mathcal{C}_1:=(\us_1,\cM_{\us})$
  %%sg aggiunta riga seguente
  of $\cSi_1$ and $\mathcal{C}_1:=(\us_1,\cM_{\us})$ of $\cSi_2$ 
  satisfying the following properties:
 \begin{description}
 \item[-] for every $\us_1$, there exists $\us_2$ such that $R(\cC_1, \cC_2)$
   holds (and vice versa);
 \item[-] if $R(\cC_1,\cC_2)$, then $\cM_{\us_1} \models \iota_1(\us_1)$ iff
   $\cM_{\us_2} \models \iota_2(\us_2)$;
 \item[-] if $R(\cC_1,\cC_2)$ and $\cM_{\us_1}\models \tau(\us_1, \us'_1)$ (for some configuration $\cC'_1:=(\us'_1,\cM_{\us'_1}))$, then
   there exist $\cC'_2$ and $n\geq 0$ such that $R(\cC'_1, \cC'_2)$ and
   $\cM_{\us_2}\models \tau^n(\us_2, \us'_2)$ (and vice versa).
 \end{description}
 The safety problems $(\cSi_1, \upsilon_1)$ and $(\cSi_2, \upsilon_2)$ are
 \emph{compatible with the bisimulation $R$} iff $R(s_1,s_2)$ implies
 that $\cM_{\us_1} \models \upsilon_1(\us_1)$ iff $\cM_{\us_2} \models \upsilon_2(\us_2)$.
\end{definition}

Let us call $\exists\forall$-formulae the formulae of the kind %AG: it should be the $\exists\forall
\begin{equation}\label{eq:s02}
\exists \ue\; \forall \ui \; \phi(\ue, \ui, \ux, \ua)
\end{equation}
where the variables $\ue, \ui$ are variables whose sort is an artifact sort and $\phi$ is quantifier-free. Notice that the only allowed \emph{universally} quantified variables in $\exists\forall$-formulae are all of artifact sorts.



The following key property for bisimulations of Universal RASs is
an immediate consequence of the fact that symbolic unsafe traces (i.e., Formulae~\eqref{eq:smc1}) in
the definition of the safety problem are $\exists\forall$-formulae and that a
$\exists\forall$-formula is satisfiable in a generic DB-instance  iff it is
satisfiable in DB-instance where each artifact relation is a finite set\footnote{this fact follows trivially by the definitions since artifact sorts are not target of any function symbol, but it is also explicitly noticed in an analogous but slightly different context in \cite{jsat})}.
\begin{lemma}
  \label{lem:bisim}
  Suppose that $R$ is a bisimulation between $\cSi_1=\tup{\Sigma,T,\ext{\Sigma}, \ux, \ua,  \iota_1,\tau_1}$
  and $\cSi_2=\tup{\Sigma,T,\ext{\Sigma}, \ux, \ua,  \iota_2,\tau_2}$ and that the safety problems $(\cSi_1,
  \upsilon_1)$ and $(\cSi_2, \upsilon_2)$ are compatible with $R$.  Then, $\cSi_1$
  is safe with respect to $\upsilon_1$ iff $\cSi_2$ is safe with respect to
  $\upsilon_2$.
\end{lemma}


\begin{proof}
	%Recall that $\mathcal S$ is unsafe iff there is
	%no DB-instance $\cM$ of $\tup{\ext{\Sigma}, T}$, no $k\geq 0$ and no assignment in $\cM$ to the variables $\ux^0,\ua^0 \dots, \ux^k, \ua^k$ such that the formula~\eqref{eq:smc1}
	First of all, we show the claim that a symbolic unsafe trace is a  $\exists\forall$-formula.
	Then,  we exploit the fact that an $\exists\forall$-formula is satisfiable in a DB-instance $\cM$ of $\tup{\ext{\Sigma}, T}$ iff it is
satisfiable in DB-instance $\cM'$ of $\tup{\ext{\Sigma}, T}$ where, for every $\mathcal{S} \in \ext{\Sigma}$, $\mathcal{S}^{\cM'}$ is a finite set: indeed, thanks to the claim, symbolic unsafe traces are $\exists\forall$-formulae, hence we can just focus on configurations in order to detect safety. This shows that the compatibilty (with a bisimilation $R$) implies the equivalence of the safety problems.

Let us now prove the claim.
 Suppose we have a symbolic unsafe trace (Formula~\eqref{eq:smc1}):
	\[
	\iota(\ux^0, \ua^0) \wedge \tau(\ux^0,\ua^0, \ux^1, \ua^1) \wedge \cdots \wedge\tau(\ux^{k-1},\ua^{k-1},
	\ux^k,\ua^{k})\wedge \upsilon(\ux^k,\ua^{k})
	\]
	that is true in a DB-instance $\cM$ of $\tup{\ext{\Sigma}, T}$, under some assignment ${\tt a}$ in $\cM$.  	
	%It is sufficient to show that this is equivalent to saying that there is
	%no $\ext{\Sigma}$-model $\cM$ of $T^*$, no $k\geq 0$ and no assignment in $\cM$ to the variables $\ux^0,\ua^0 \dots, \ux^k, \ua^k$ such that~\eqref{eq:smc1} is true in $\cM$
	%(once this is shown, the proof goes in the same way as the proof of Theorem~\ref{thm:basic}).
	
	Now, the Formula~\eqref{eq:smc1} is satisfiable in a $\ext{\Sigma}$-structure $\cM$ under a suitable assignment iff the formula
	\begin{eqnarray*}
		%\exists \ua^0\exists \ux^0(
		\iota(\ux^0, \ua^0) ~~\wedge
		& \exists \ua^1\exists\ux^1 (\tau(\ux^0,\ua^0, \ux^1, \ua^1) \wedge \cdots ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
		\\ &
		\cdots
		\wedge \exists \ua^k\exists \ux^k(\tau(\ux^{k-1},\ua^{k-1},
		\ux^k,\ua^{k})\wedge \upsilon(\ux^k,\ua^{k}))\cdots)
		%)
	\end{eqnarray*}
	is satisfiable in $\cM$ under a suitable assignment. We now show that the latter is equivalent to a formula of the kind
	\begin{equation}\label{eq:forall-exist-new}
	\iota(\ux, \ua)~\wedge~\exists \ue\,\exists \uy\,(\phi(\ue,\uy,\ux, \ua)\land \forall k  \; \psi(k,\ue,\uy,\ux, \ua))
	\end{equation}
	where $\phi$ and $\psi$ are quantifier-free, the $\ue$
	are variables of artifact sorts and the $\uy$ are variables of  basic sorts  (we renamed $\ux^0, \ua^0$ as $\ux, \ua$).
	
	 We manipulate the formula
	\begin{equation}\label{eq:pre-new-lemma}
	\exists \ux'\,\exists \ua'\, (\tau(\ux, \ua, \ux', \ua') \wedge \exists \ue~ \phi(\ue, \ux',\ua'))
	\end{equation}
	%AG: shouldn't "conjunction" be "disjunction"?
	up to logical equivalence, where $\tau$ is given by\footnote{Actually, $\tau$ is a disjunction of such formulae, but it easily seen that disjunction can be
		accommodated by moving existential quantifiers back-and-forth through them.}
	\begin{equation*}
	\exists \ue_0\left(\gamma(\ue_0, \ux, \ua) \wedge (\forall k  \; \gamma_u(k,\ue,\uy,\ux, \ua)) \wedge 
	\ux'= \uF(\ue_0, \ux, \ua) \wedge \ua'=\lambda y. \uG(y,\ue_0,\ux, \ua)
	\right)
	\end{equation*}
	(here we used plain equality  for conjunctions of equalities, e.g. $\ux'= \uF(\ue_0, \ux, \ua)$ stands for $\bigwedge_i x'_i= F_i(\ue, \ux, \ua)$).
	Repeated substitutions  show that~\eqref{eq:pre-new-lemma} is equivalent to
	\begin{equation*}
	\exists \ue\,\exists \ue_0\, \left(\gamma(\ue_0, \ux, \ua) \wedge (\forall k  \; \gamma_u(k,\ue,\uy,\ux, \ua)) \wedge \phi(\ue, \uF(\ue_0, \ux,\ua)/\ux',\lambda y.\uG(y,\ue_0,\ux, \ua)/\ua' )\right)
	\end{equation*}
	which is a formula of the required format.
	% $\hfill\dashv$
	
	Hence, the Formula~\eqref{eq:smc1} is satisfiable in a $\ext{\Sigma}$-structure $\cM$ under a suitable assignment iff  a formula of the kind~\eqref{eq:forall-exist-new} is satisfiable in a $\ext{\Sigma}$-structure $\cM$ under a suitable assignment. 
	 	
	However, the satisfiability of~\eqref{eq:forall-exist-new} is clearly the same as the satisfiability of
	%sg 26/6/18 cambiato qui
	$\exists \ue\,(\iota(\ux,\ua) \wedge\phi(\ue,\uy,\ux, \ua)  \wedge \forall k  \; (\psi(k,\ue,\uy,\ux, \ua)))$; %AG:25july ho sostituito le z con le y, come richiesto dal referee per rendere uniforme la notazione con il lemma 4.2
	the latter, in view of~\eqref{eq:ini1}, has the following format:
	
	$$\exists \ue\,\left((\bigwedge_{i=1}^n x_i= c_i) \land  \forall k_1 \; (\bigwedge_{j=1}^m a_j[k_1] = d_j) \wedge\phi(\ue,\uy,\ux, \ua)  \wedge \forall k  \; (\psi(k,\ue,\uy,\ux, \ua))\right)$$. Pushing the universal quantifiers in front of the formula, we get:
	%
	$$\exists \ue\,\forall k_1, k \; \left((\bigwedge_{i=1}^n x_i= c_i) \land  \; (\bigwedge_{j=1}^m a_j[k_1] = d_j) \wedge\phi(\ue,\uy,\ux, \ua)  \wedge \; (\psi(k,\ue,\uy,\ux, \ua))\right)$$.
	 %
	which is a $\exists\forall$-formula, as wanted.
	\end{proof}

The following proposition states that the safety problems for $\tilde \cSi$ and $\widehat{\cSi}$ are equivalent.
\begin{proposition}
  \label{prop:result-abstract}
  %%% SRlast: I have slightly simplified the statement of the
  %%% theorem... 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  Let $\cSi=\tup{\Sigma,T,\ext{\Sigma}, \ux, \ua,  \iota,\tau}$ be a Universal RAS and $(\cSi, \upsilon)$ be a
  safety problem for it.  %% , where $\cSi=(a,I,\tau)$---notice that we assume that $\tau$ may
  %% contain disjuncts of the form (\ref{eq:transition3}).
  Then, $\tilde \cSi$
  is safe with respect to $\tilde \upsilon$ iff $\widehat{\cSi}$ is safe with
  respect to $\widehat{\upsilon}$.
\end{proposition}
\begin{proof}
% FA - RW2 - Lemma 5.6 above --> Lemma 5.6
  We apply Lemma~\ref{lem:bisim} with the identity relation as
  the bisimulation.  The proof can be concluded by observing that the
  transition $\widehat{\tau}$ can be simulated by finitely many applications
  of the additional transition $\tilde{\univtrans}_{r+1}$ in the intermediate
 Universal RAS of Table~\ref{tab:transformation1} followed by a single
  application of $\tilde \tau$;
% FA - RW2 - vice versa --> conversely
  conversely, each application of
  $\tilde \tau$ is obviously also an application of $\widehat{\tau}$.
\end{proof}

The importance of
% FA - RW2 - the above Theorem 5.7 --> Theorem 5.7
Proposition~\ref{prop:result-abstract} lies in the fact that the transition
$\widehat{\tau}$ of $\widehat{\cSi}$  does
not have universal quantifiers in guards.  This allows us to automate
$\mathsf{BReach}_{\ras}$ over $(\widehat{\cSi}, \widehat \upsilon)$ as explained in Section~\ref{sec:safety-uras}.

We are now ready to prove the main result about the transformation from Universal RASs to RAS{s}, which is a consequence of Proposition~\ref{prop:result-abstract} and Proposition~\ref{prop:preserve-safety}:

\begin{proposition}
  \label{prop:main-result-abstract}
  Let $\cSi=\tup{\Sigma,T,\ext{\Sigma}, \ux, \ua,  \iota,\tau}$ be a Universal RAS and $\upsilon$ be an unsafe formula. Then, if the (plain) RAS $\widehat \cSi$ is safe with respect to $\widehat \upsilon$, then $\cSi$ is
  safe with respect to $\upsilon$.
  \end{proposition}

The previous proposition is significant because it partially reduces the problem of assessing safety for Universal RASs to the one of assessing safety for plain RASs. Unfortunately, this reduction is partial because when the plain RAS $\widehat \cSi$ is unsafe w.r.t. $\widehat \upsilon$, nothing can be established for the original Universal RAS $\cSi$. If we are able to show that $\mathsf{BReach}_{\ras}$ is sound for checking unsafety of \ras{s}, then we conclude, thanks to the previous observations, that we can still run $\mathsf{BReach}_{\ras}$ over $(\widehat{\cSi}, \widehat \upsilon)$, with $\cSi$ Universal RAS: in case we find out that the output is \safe, we can conclude safety of $\cSi$ w.r.t. $\upsilon$ as well. As a side remark, we only notice (but it is out of scope of the thesis) that it can be proved, by adapting the results from \cite{invariant} to this declarative setting, that when a \emph{universal invariant} for $\cS$ w.r.t. the unsafe formula $\upsilon$ exists, backward search cannot terminate with an \unsafe outcome, so in this case no spurious trace can be found.

The following section is devoted to attack the problem of verifying safety of plain RASs via  $\mathsf{BReach}_{\ras}$ and showing that this procedure is sound for checking safety of $\mathsf{BReach}_{\ras}$.



\endinput 


\subsection{Invariants and relativization of quantifiers}
\label{subsec:inv-and-relativization}

It is well-known that invariants can dramatically prune the search
space of backward reachability procedures; see~\cite{tableaux09,lmcs}
for an in-depth discussion about this issue and related experiments.
Here, we briefly recall the notion of invariant for array-based
systems and explain how they can be used in combination with the
technique for eliminating universal conditions from guards.

A $\forall^I$-formula $\forall \ui\, \phi(\ui, a[\ui])$ is an
\emph{(inductive) invariant} for an array-based system
$\cSi=(a,I,\tau)$ iff the formulae (a) $I \Rightarrow \forall \ui\,
\phi(\ui, a[\ui])$ and (b) $\forall \ui\, \phi(\ui, a[\ui])\wedge
\tau(a, a') \Rightarrow \forall \ui\, \phi(\ui, a'[\ui])$ are both
$A^E_I$-valid. If, in addition to (a) and (b), also the formula (c)
$\forall \ui\, \phi(\ui, a[\ui])\wedge U(a)$ is $A^E_I$-unsatisfiable,
then we say that the $\forall^I$-formula $\forall \ui\, \phi(\ui,
a[\ui])$ is a \emph{safety invariant} for the safety problem
$(\cSi,U)$.  Notice that the $A^E_I$-validity and
$A^E_I$-satisfiability tests required in (a), (b), and (c) are
decidable by Theorem~\ref{th:decidability} under the hypothesis
\textbf{(HT1)}, \textbf{(HT2)}, \textbf{(HF1)}, \textbf{(HF2)}, and
\textbf{(wHF3)} in Table~\ref{tab:assumptions}.  Thus, in a sense,
using invariant for the verification of safety properties---called the
\emph{invariant method} in the literature---is more general than using
a backward reachability procedure as we propose in
Section~\ref{sec:array}.  Unfortunately, the invariant method is more
difficult to apply because finding safety invariants cannot be
mechanized (see again~\cite{tableaux09,lmcs} for details).
%%sg-last c'era già un 'unfortunately' poco sopra 
%Fortunately, 
However,
if an invariant has been found in some way (for instance,
by using some heuristics) or it is supplied by a trusted third-party,
the invariant can be put to productive use (even if it is not a safety
invariant) in the backward reachability procedure by adding it as an
extra hypothesis in the fix-point test.  More precisely, line 2 of
$\mathsf{Breach}$ in Figure~\ref{fig:reach-algo} can be substituted by
the following instruction:
\begin{quote}
  \centering
  2$'$ \textbf{while} ($P\wedge \mathit{Inv}\wedge \neg B$ is $A^E_I$-sat.) \textbf{do}
\end{quote}
where $Inv$ is a conjunction of the available invariants, i.e.\
$\forall^I$-formulae satisfying conditions (a) and (b) above.  In this
way, we try to augment the possibility to detect unsatisfiability by
% FA - RW2 - furtherly --> further 
further constraining the formula $P\wedge \neg B$ with the
invariants in $\mathit{Inv}$.  As shown in~\cite{tableaux09,lmcs},
this modification may have dramatic effects on the performance of the
backward reachability procedure; in some cases, we may even get a
safety certificate by using invariants while the procedure does not
terminate without them.

Combining invariants with the technique for eliminating universal
conditions in guards described above is straightforward; it is
sufficient to relativize the universal quantifiers occurring in
$\forall^I$-formulae.  More precisely, we extend the mapping
$(\tilde{\cdot})$ to invariants as follows:
\begin{eqnarray*}
  \forall \ui\, \phi(\ui, a[\ui]) & \longmapsto &
  \forall \ui\, ({\tt A}(\ui)\Rightarrow \phi(\ui, a[\ui]) )
\end{eqnarray*}
where ${\tt A}$ is defined as in Table~\ref{tab:transformation}.  The
mapping $(\hat{\cdot})$ acts as the identity on invariants.  It is
easy to adapt the results of
Sections~\ref{subsec:props-relativization}
and~\ref{subsec:props-for-+} for the two mappings extended in this
way.




